Beyond Empirical Windowing: An Attention-Based Approach for Trust Prediction in Autonomous Vehicles

Humans' internal states play a key role in human-machine interaction, leading to the rise of human state estimation as a prominent field. Compared to swift state changes such as surprise and irritation, modeling gradual states like trust and satisfaction are further challenged by label sparsity: long time-series signals are usually associated with a single label, making it difficult to identify the critical span of state shifts. Windowing has been one widely-used technique to enable localized analysis of long time-series data. However, the performance of downstream models can be sensitive to the window size, and determining the optimal window size demands domain expertise and extensive search. To address this challenge, we propose a Selective Windowing Attention Network (SWAN), which employs window prompts and masked attention transformation to enable the selection of attended intervals with flexible lengths. We evaluate SWAN on the task of trust prediction on a new multimodal driving simulation dataset. Experiments show that SWAN significantly outperforms an existing empirical window selection baseline and neural network baselines including CNN-LSTM and Transformer. Furthermore, it shows robustness across a wide span of windowing ranges, compared to the traditional windowing approach.

==> copies.tex <==
% ---------------- discussion + conclusion from Kevin-------------------
This research propose AWAN, adaptive windowing attention network, that utilizes range masks for adaptive window selection and weighting. We applied AWAN on driver trust prediction as a case study, to investigate the efficiency of such model to extract critical moments, that triggers changes in prolonged driver states. We collected a multimodal dataset through a SAE Level 2 driving simulator, with a total of 48 participants. Participants observed traffic events on an automated mobility, and self rated their trust in the automation after each traffic event. Then, we used a random forest classifier, a CNN-LSTM network, and the proposed AWAN to predict participants' trust levels. The proposed AWAN significantly outperformed the RF and CNN-LSTM baseline. To further demonstrate the efficiency of AWAN, we compared the baseline performance and AWAN performance on various lengths of time windows. The experiment results show that AWAN is very adaptive to window length change, that its performance has negligible variation on a wide range of window lengths. At the same time, RF baseline performance show randomly varying changes, which is consistent with existing research. We also visualize the attention weight of AWAN with traffic events. It is observed that AWAN could identify crucial intervals, that are more related to high-intensity interactions during travel events. Thus, AWAN may provide a novel solution to model prolonged driver internal state with multimodal time-series signals, that is more accurate, lightweight, and interpretable. 

Despite the potential, this research has some limitations. First, the sample size of the collected dataset is small and imbalanced, that limits the network complexity of AWAN. With more time and resources, more data collected would further test the efficiency of the proposed network. Secondly, we applied AWAN on driver trust prediction, and there are more driver state of interest, such as fatigue and reliance. For potential future work, we could use AWAN for other driver state estimation tasks and potentially with public dataset, to explore how generalized AWAN is for prolonged driver state estimation. As a conclusion, this work provide a novel solution to model prolonged driver internal state with multimodal time-series signals. Its robustness across a diverse spectrum of window range potentially revolute the tedious process of window size selection.




% --------------------------- Intro, first draft --------------------------
\section{Introduction}
\label{sec:intro}
Autonomous vehicle (AV) and advanced driver assistance systems (ADAS) provide potential benefits in fuel efficiency, user convenience, and safety~\cite{beza2019potential, zhu2019automated}. Despite the remarkable trend in mobility industry to further develop and deploy AV and ADAS, trust in automation remains a key factor for user acceptance~\cite{nordhoff2019multi}. Proper trust can lead to more frequent employment of AV or ADAS systems~\cite{molnar2018understanding}, and reduce driver anxiety~\cite{kraus2020scared}. Trust in automation is also correlated with the preferred driving style of the AV~\cite{zheng2022identification}. Thus, trust calibration and monitoring play a key part in human-automation interaction~\cite{hu2016real}. 

Prediction of driver state in automation through multimodal sensing has emerged, to provide an automatic and continuous driver monitoring. Akash et al. used electroencephalogram (EEG) and galvanic skin responses (GSR) to sense trust~\cite{akash2017dynamic}. They built a customized trust sensor model, using selected features for each individual, that resulted in improved mean accuracy than the general model. Ayoub et al. used eye gaze, GSR, and heart rate (HR) to predict trust in conditionally automated vehicles~\cite{ayoub2022real}. They applied a Gradient Boosting framework for its robustness to over-fitting and missing data points. Yi et al. used a CNN-LSTM network to recognize driver trust in conditionally automated vehicles~\cite{yi2023measurement}. Their real-time sensing modalities include GSR, HR, and eye gaze. Yu et al. investigated driver trust prediction with hand position transition probability matrix~\cite{yu2021measurement}. The hand position matrix showed strong correlation with the self-rated trust levels. These related work implicate the feasibility of in-vehicle trust monitoring systems, that can actively facilitate human-AV interaction. 

Despite the demonstrated potential, a key challenge of driver state modeling task remains to learn from long time-series input and sparse behavioral labels~\cite{poria2017review}. Over an extended period following the establishment of a user's familiarity with the vehicle, trust tends to remain generally stable, with alterations happen at some critical moments triggered by specific events~\cite{ekman2017creating}. Frequent surveys are also a major distraction to participants and may cause fatigue, resulting in sparse labels of driver state labels~\cite{porter2004multiple}. Therefore, models need to learn to identify those critical moments from long, noisy time-series input. Windowing is one of the most common approach to tackle this challenge, which has been effective on many tasks~\cite{akash2018classification}. However, empirical window selection is time extensive and not thorough. Existing window selection work on multimodal learning has revealed that the optimal window length for each feature may not be static~\cite{konishi2022inferring}. The optimal window may be dependent on feature type, individual responses, and contextual information, and thus it takes domain expertise and extensive search attempts to find the optimal windows. Recently, deep neural networks such as Convolutional Neural Networks (CNN) and Transformer have been used more in driver state detection signal processing~\cite{koochaki2023learn}. They outperformed traditional methods in many tasks, but they are heavily data-dependent and unexplained on the network behavior, and thus interpretation of the cause of human state change remain unclear.
% maybe add in the future: Transformers are not good at modeling long time serie\cite{zeng2023transformers}

Therefore, we propose Adaptive Windowing Attention Network (AWAN), as an automatic windowing process while enabling flexible-length attended area selection through gradient-based optimization. In summary, the contributions of the study are as follows: 1) an end-to-end attention network that learns directly from time-series data, and assigns attention to critical areas; 2) analysis on the machine learning results to demonstrate the model adaptability over long time spans, and interpret model attention on traffic events; 3) a public dataset with multimodal time-series signals and user trust labels.
% trust labels, and multimodal human signals. 
% 1) it allows learning from time-series data, without feature extraction; 2) it automatically identifies critical areas and assign more attention to them; 3) compare to Transformers or CNN, it's light-weight and requires much less data to train; 4) The number of parameters doesn't scale as the windows grow, making it more suitable to capture trends over longer time spans or signals of higher frequencies. 

% intro, second draft
With the advance of wearable sensing and machine learning, there has been existing work on 
Autonomous vehicle (AV) and advanced driver assistance systems (ADAS) provide potential benefits in fuel efficiency, user convenience, and safety~\cite{beza2019potential, zhu2019automated}. 
% Despite the remarkable trend in mobility industry to further develop and deploy AV and ADAS, trust in automation remains a key factor for user acceptance~\cite{nordhoff2019multi}. 
Beyond the remarkable effort of the mobility industry in enhancing the driving capabilities of self-driving technologies, it is also important to consider and model users' internal states. Users' emotional and cognitive conditions deeply influence how they interact with vehicles, and thus is closely connected to safety, system efficiency and user experience.
Proper trust can lead to more frequent employment of AV or ADAS systems~\cite{molnar2018understanding}, and reduce driver anxiety~\cite{kraus2020scared}. Trust in automation is also correlated with the preferred driving style of the AV~\cite{zheng2022identification}. Thus, user state calibration and monitoring play a key part in human-automation interaction~\cite{hu2016real}. 

Prediction of driver state in automation through multimodal sensing has emerged, to provide automatic and continuous driver monitoring. Akash et al. used electroencephalogram (EEG) and galvanic skin responses (GSR) to sense trust~\cite{akash2017dynamic}. They built a customized trust sensor model, using selected features for each individual, that resulted in improved mean accuracy than the general model. Ayoub et al. used eye gaze, GSR, and heart rate (HR) to predict trust in conditionally automated vehicles~\cite{ayoub2022real}. They applied a Gradient Boosting framework for its robustness to over-fitting and missing data points. Yi et al. used a CNN-LSTM network to recognize driver trust in conditionally automated vehicles~\cite{yi2023measurement}. Their real-time sensing modalities include GSR, HR, and eye gaze. Yu et al. investigated driver trust prediction with hand position transition probability matrix~\cite{yu2021measurement}. The hand position matrix showed strong correlation with the self-rated trust levels. These related work implicate the feasibility of in-vehicle trust monitoring systems, that can actively facilitate human-AV interaction. 

Despite the demonstrated potential, a key challenge of driver state modeling task remains to learn from long time-series input and sparse behavioral labels~\cite{poria2017review}. Over an extended period following the establishment of a user's familiarity with the vehicle, trust tends to remain generally stable, with alterations happen at some critical moments triggered by specific events~\cite{ekman2017creating}. Frequent surveys are also a major distraction to participants and may cause fatigue, resulting in sparse labels of driver states~\cite{porter2004multiple}. Therefore, models need to identify those critical moments from long, noisy time-series input. 

Windowing has been one of the most common techniques to tackle this challenge~\cite{akash2018classification}. It enables localized analysis through the segmentation of a prolonged sequence into fixed-size, often overlapping intervals. Yet, empirical window selection is non-trivial. Existing window selection work on multimodal learning has revealed that the optimal window length for each feature may not be static~\cite{konishi2022inferring}. The optimal window may be dependent on feature type, individual responses, and contextual information, and thus it takes domain expertise and extensive search attempts to find the optimal windows. Recently, Deep Neural Networks such as Convolutional Neural Networks (CNN) and Transformers have gained traction in multimodal signal processing~\cite{kiranyaz20191, wen2022transformers}. They outperformed traditional methods in many tasks, but their training usually requires large training set, which is often not available in datasets with human state labels.
% but they are heavily data-dependent and unexplained on the network behavior, and thus interpretation of the cause of human state change remain unclear.
% maybe add in the future: Transformers are not good at modeling long time serie\cite{zeng2023transformers}

Therefore, we propose Adaptive Windowing Attention Network (AWAN), an automatic windowing network which enables flexible-length attended area selection through gradient-based optimization. In summary, the contributions of the study are as follows: 1) an end-to-end attention network that learns directly from time-series data, and assigns attention to critical areas; 2) analysis on the machine learning results to demonstrate the model adaptability over long time spans, and interpret model attention on traffic events; 3) a public dataset with multimodal time-series signals and user trust labels.
% trust labels, and multimodal human signals. 
% 1) it allows learning from time-series data, without feature extraction; 2) it automatically identifies critical areas and assign more attention to them; 3) compare to Transformers or CNN, it's light-weight and requires much less data to train; 4) The number of parameters doesn't scale as the windows grow, making it more suitable to capture trends over longer time spans or signals of higher frequencies.
